Learning State Abstractions for Transfer in Continuous Control

Can simple algorithms with a good representation solve challenging reinforcement learning problems? In this work, we answer this question in the affirmative, where we take "simple learning algorithm" to be tabular Q-Learning, the "good representations" to be a learned state abstraction, and "challenging problems" to be continuous control tasks. Our main contribution is a learning algorithm that abstracts a continuous state-space into a discrete one. We transfer this learned representation to unseen problems to enable effective learning. We provide theory showing that learned abstractions maintain a bounded value loss, and we report experiments showing that the abstractions empower tabular Q-Learning to learn efficiently in unseen tasks.

==> other.tex <==

\section{Other Ideas}

Another iterative optimization process could be to jointly optimize over a clustering and a set of options. That is, first you pick a clustering, then subject to that clustering you pick a set of options, and so on.




==> proofs/pol_similarity_abstr_exp_val_loss.tex <==
\begin{proof}
Our goal is to bound:
\begin{equation}
    \bE_{s \sim \mu^{\pi_d}(s)} \left[V^d(s) - V^\phi(s) \right],
\end{equation}
as a function of $\eps$, the known (maximum) gap between policies in each abstract state. \\


We proceed by induction.

Specifically, we define a policy that changes from $\pi_\phi$ to $\pi_d$ after $t$ steps, $\pi_{\phi,d}^{t,i}$. Here $t$ is the inductive parameter, and $i$ denotes the number of steps the policy has taken from a particular state. The policy is defined as follows, for a given state $s$:
\begin{equation}
   \pi_{\phi,d}^{t,i}(s) = \begin{cases}
   \pi_\phi(s)&i \leq t \\
   \pi_d(s)&i > t \\
   \end{cases}
\end{equation}

Thus, when we have followed the policy for $\leq t$ steps, we follow the abstract policy $\pi_\phi$. Thereafter, we follow $\pi_d$.

We proceed by induction on $t$. \\


{\it Base Case ($t = 0$):} \\

When $t = 0$, the hybrid policy is trivially the same as $\pi_d$ for all $t$. \\

\spacerule

{\it Inductive Case ($t > 0$):} \\

When $t > 0$, we define the inductive hypothesis as follows:

\begin{equation}
    \bE_{s \sim \mu^d} \left[V^d(s) - V^{\pi_{\phi,d}^{t,i}}\right] \leq \sum_{i=1}^t \gamma^i \eps
    \tag{IH}
\end{equation}

We now endeavor to show that 
\begin{equation}
    \bE_{s \sim \mu^d} \left[V^d(s) - V^{\pi_{\phi,d}^{t+1,i}}\right] \leq \sum_{i=1}^{t+1} \gamma^i \eps
\end{equation}



\end{proof}
